Bayesian Quantile Regression with Subset Selection: A Decision Analysis Perspective

Quantile regression is a powerful tool for inferring how covariates affect specific percentiles of the response distribution. Existing methods either estimate conditional quantiles separately for each quantile of interest or estimate the entire conditional distribution using semi- or non-parametric models. The former often produce inadequate models for real data and do not share information across quantiles, while the latter are characterized by complex and constrained models that can be difficult to interpret and computationally inefficient. Neither approach is well-suited for quantile-specific subset selection. Instead, we pose the fundamental problems of linear quantile estimation, uncertainty quantification, and subset selection from a Bayesian decision analysis perspective. For any Bayesian regression model -- including, but not limited to existing Bayesian quantile regression models -- we derive optimal point estimates, interpretable uncertainty quantification, and scalable subset selection techniques for all model-based conditional quantiles. Our approach introduces a quantile-focused squared error loss that enables efficient, closed-form computing and maintains a close relationship with Wasserstein-based density estimation. In an extensive simulation study, our methods demonstrate substantial gains in quantile estimation accuracy, inference, and variable selection over frequentist and Bayesian competitors. We use these tools to identify and quantify the heterogeneous impacts of multiple social stressors and environmental exposures on educational outcomes across the full spectrum of low-, medium-, and high-achieving students in North Carolina.

==> arXivVersionaux.tex <==
%% LaTeX2e file `arXivVersionaux'
%% generated by the `filecontents' environment
%% from source `supplement' on 2024/11/16.
%%
\relax
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyperFirstAtBeginDocument{\AtBeginDocument}
\HyperFirstAtBeginDocument{\ifx\hyper@anchor\@undefined
\global\let\oldnewlabel\newlabel
\gdef\newlabel#1#2{\newlabelxx{#1}#2}
\gdef\newlabelxx#1#2#3#4#5#6{\oldnewlabel{#1}{{#2}{#3}}}
\AtEndDocument{\ifx\hyper@anchor\@undefined
\let\newlabel\oldnewlabel
\fi}
\fi}
\global\let\hyper@last\relax
\gdef\HyperFirstAtBeginDocument#1{#1}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\citation{kottas2001bayesian}
\citation{bassett2002portfolio}
\citation{pandey1999comparative}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{2}{section.1}\protected@file@percent }
\newlabel{linearQR}{{1}{2}{Introduction}{equation.1.1}{}}
\citation{koenker1978regression}
\citation{koenker2017handbook}
\citation{yu2001bayesian}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.1}Separate Quantile Regressions}{4}{subsection.1.1}\protected@file@percent }
\newlabel{sec-sep}{{1.1}{4}{Separate Quantile Regressions}{subsection.1.1}{}}
\newlabel{CL}{{2}{4}{Separate Quantile Regressions}{equation.1.2}{}}
\citation{ALconsist}
\citation{kozumi2011gibbs,fasiolo2021fast}
\citation{benoit2017bayesqr,alhamzawi2020brq}
\citation{kowal2024monte}
\newlabel{AL}{{3}{5}{Separate Quantile Regressions}{equation.1.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.2}Simultaneous Quantile Regression Methods}{5}{subsection.1.2}\protected@file@percent }
\newlabel{simult}{{1.2}{5}{Simultaneous Quantile Regression Methods}{subsection.1.2}{}}
\citation{bondell2010noncrossing}
\citation{Tokdar}
\citation{emplike}
\citation{dunson2005approximate}
\citation{kottas2001bayesian,kottas2009bayesian,reichBNPqr,reich2013bayesian}
\citation{taddy2010bayesian}
\citation{wu2009variable,10.1214/10-AOS827,wang2012quantile,lee2014model}
\citation{DKJMLR}
\citation{furnival2000regressions,hofmann2007efficient,Bertsimas2006}
\citation{li20081,alhamzawi2012bayesian,chen2013bayesian,keil2020quantile,dao2022bayesian}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.3}Subset Selection in Quantile Regression}{7}{subsection.1.3}\protected@file@percent }
\citation{pratola2020heteroscedastic}
\citation{raftery1997bayesian}
\citation{stacking}
\citation{frechet1948elements}
\@writefile{toc}{\contentsline {subsection}{\numberline {1.4}Overview of the Proposed Approach}{8}{subsection.1.4}\protected@file@percent }
\@writefile{loa}{\contentsline {algorithm}{\numberline {1}{\ignorespaces Bayesian decision analysis for quantile regression\relax }}{9}{algorithm.1}\protected@file@percent }
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{alg1}{{1}{9}{Bayesian decision analysis for quantile regression\relax }{algorithm.1}{}}
\citation{HahnCarvalho,woody,kowal2021fast,DKJMLR}
\@writefile{toc}{\contentsline {section}{\numberline {2}Bayesian Decision Analysis for Quantile Regression}{10}{section.2}\protected@file@percent }
\newlabel{sec1}{{2}{10}{Bayesian Decision Analysis for Quantile Regression}{section.2}{}}
\newlabel{LLS}{{4}{11}{Bayesian Decision Analysis for Quantile Regression}{equation.2.4}{}}
\newlabel{QF}{{5}{11}{Bayesian Decision Analysis for Quantile Regression}{equation.2.5}{}}
\newlabel{post-dec}{{6}{12}{Bayesian Decision Analysis for Quantile Regression}{equation.2.6}{}}
\newlabel{relax-wass}{{7}{12}{Bayesian Decision Analysis for Quantile Regression}{equation.2.7}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.1}Point Estimation for Linear Quantiles}{12}{subsection.2.1}\protected@file@percent }
\newlabel{LinActions}{{2.1}{12}{Point Estimation for Linear Quantiles}{subsection.2.1}{}}
\newlabel{OLS}{{2.1}{12}{}{theorem.2.1}{}}
\newlabel{OLS_sol}{{8}{13}{}{equation.2.8}{}}
\newlabel{cor1}{{1}{13}{}{corollary.1}{}}
\newlabel{cor2}{{2}{14}{}{corollary.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.2}Posterior Uncertainty Quantification}{14}{subsection.2.2}\protected@file@percent }
\newlabel{projecting}{{2.2}{14}{Posterior Uncertainty Quantification}{subsection.2.2}{}}
\newlabel{proj}{{9}{15}{Posterior Uncertainty Quantification}{equation.2.9}{}}
\newlabel{cor3}{{3}{15}{}{corollary.3}{}}
\citation{PetersenAlexander2021W}
\citation{PetersenAlexander2021W}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.3}Connection with the Wasserstein Geometry}{16}{subsection.2.3}\protected@file@percent }
\newlabel{wass}{{2.3}{16}{Connection with the Wasserstein Geometry}{subsection.2.3}{}}
\newlabel{sqwass}{{10}{16}{Connection with the Wasserstein Geometry}{equation.2.10}{}}
\newlabel{wass_int}{{11}{16}{Connection with the Wasserstein Geometry}{equation.2.11}{}}
\newlabel{emp-wass}{{12}{17}{Connection with the Wasserstein Geometry}{equation.2.12}{}}
\newlabel{post-dec-density}{{13}{17}{Connection with the Wasserstein Geometry}{equation.2.13}{}}
\newlabel{form_relax_wass}{{2.2}{17}{}{theorem.2.2}{}}
\citation{woody}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.4}Extensions for Nonlinear Quantiles}{18}{subsection.2.4}\protected@file@percent }
\newlabel{sec-nl}{{2.4}{18}{Extensions for Nonlinear Quantiles}{subsection.2.4}{}}
\citation{kowal2021fast}
\@writefile{toc}{\contentsline {section}{\numberline {3}Quantile-Specific Subset Search and Selection}{19}{section.3}\protected@file@percent }
\newlabel{subset search}{{3}{19}{Quantile-Specific Subset Search and Selection}{section.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1}Subset Search with Decision Analysis}{19}{subsection.3.1}\protected@file@percent }
\newlabel{exp-loss}{{14}{19}{Subset Search with Decision Analysis}{equation.3.14}{}}
\newlabel{post-loss}{{15}{19}{Subset Search with Decision Analysis}{equation.3.15}{}}
\citation{furnival2000regressions,hofmann2007efficient,Bertsimas2006}
\citation{furnival2000regressions}
\citation{kowal2021fast,DKJMLR}
\citation{kowal2021fast}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2}Subset Filtration}{21}{subsection.3.2}\protected@file@percent }
\newlabel{filt}{{3.2}{21}{Subset Filtration}{subsection.3.2}{}}
\newlabel{post-dif}{{16}{21}{Subset Filtration}{equation.3.16}{}}
\newlabel{accept}{{17}{21}{Subset Filtration}{equation.3.17}{}}
\newlabel{smallest}{{18}{21}{Subset Filtration}{equation.3.18}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.3}Quantifying Variable Importance}{22}{subsection.3.3}\protected@file@percent }
\newlabel{Vimps}{{3.3}{22}{Quantifying Variable Importance}{subsection.3.3}{}}
\newlabel{VI}{{19}{22}{Quantifying Variable Importance}{equation.3.19}{}}
\@writefile{toc}{\contentsline {section}{\numberline {4}Simulation Study}{23}{section.4}\protected@file@percent }
\newlabel{sim}{{4}{23}{Simulation Study}{section.4}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.1}Simulation Design}{23}{subsection.4.1}\protected@file@percent }
\newlabel{DGP}{{20}{23}{Simulation Design}{equation.4.20}{}}
\citation{carpenter2017stan}
\newlabel{M}{{21}{24}{Simulation Design}{equation.4.21}{}}
\citation{wu2009variable}
\citation{sherwood2017rqpen}
\citation{alhamzawi2012bayesian}
\citation{benoit2017bayesqr}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2}Quantile Prediction}{25}{subsection.4.2}\protected@file@percent }
\newlabel{pred}{{4.2}{25}{Quantile Prediction}{subsection.4.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.3}Uncertainty Quantification}{26}{subsection.4.3}\protected@file@percent }
\newlabel{uq}{{4.3}{26}{Uncertainty Quantification}{subsection.4.3}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces  \small  Quantile mean squared error (MSE; left) and check loss (right) among competing quantile regression methods; nonoverlapping notches indicate significant differences between medians, and the dashed vertical line (right) denotes $\tau $. The proposed approach ($\mbox  {S}_{small}(\tau )$) offers substantial improvements in quantile prediction relative to both frequentist and Bayesian competitors, and matches or improves upon the model-based fitted quantiles ($\mbox  {Q}_{hat}$).\relax }}{27}{figure.caption.1}\protected@file@percent }
\newlabel{Fig2}{{1}{27}{\small Quantile mean squared error (MSE; left) and check loss (right) among competing quantile regression methods; nonoverlapping notches indicate significant differences between medians, and the dashed vertical line (right) denotes $\tau $. The proposed approach ($\mbox {S}_{small}(\tau )$) offers substantial improvements in quantile prediction relative to both frequentist and Bayesian competitors, and matches or improves upon the model-based fitted quantiles ($\mbox {Q}_{hat}$).\relax }{figure.caption.1}{}}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces \small  Coverage rates and average widths of 95\% credible intervals for the posterior action \eqref  {proj} with $\mbox  {S}_{small}(\tau )$ or $\mbox  {S}_{full}$ as well as $\mbox  {AL}_{Bayes}$. The intervals for $\mbox  {S}_{small}(\tau )$ and $\mbox  {S}_{full}$ are significantly more narrow than those for $\mbox  {AL}_{Bayes}$, especially for quantiles near zero or one, and typically maintain nominal coverage. $\mbox  {S}_{small}(\tau )$ sacrifices some coverage in favor of sparsity, and thus provides the most narrow intervals.  \relax }}{28}{table.caption.2}\protected@file@percent }
\newlabel{covrates}{{1}{28}{\small Coverage rates and average widths of 95\% credible intervals for the posterior action \eqref {proj} with $\mbox {S}_{small}(\tau )$ or $\mbox {S}_{full}$ as well as $\mbox {AL}_{Bayes}$. The intervals for $\mbox {S}_{small}(\tau )$ and $\mbox {S}_{full}$ are significantly more narrow than those for $\mbox {AL}_{Bayes}$, especially for quantiles near zero or one, and typically maintain nominal coverage. $\mbox {S}_{small}(\tau )$ sacrifices some coverage in favor of sparsity, and thus provides the most narrow intervals.  \relax }{table.caption.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.4}Selection}{28}{subsection.4.4}\protected@file@percent }
\newlabel{select}{{4.4}{28}{Selection}{subsection.4.4}{}}
\@writefile{lot}{\contentsline {table}{\numberline {2}{\ignorespaces \small  True positive rates (TPR) and true negative rates (TNR) for variable selection averaged across simulations. The proposed approach ($\mbox  {S}_{small}(\tau )$) neatly balances TPR and TNR. The Bayesian competitor ($\mbox  {AL}_ {Bayes}$) is significantly underpowered due to excessively wide posterior credible intervals, while the frequentist competitor (aLASSO) often overselects variables (low TNRs). The results for the $(n,p) = (100,100)$ are qualitatively similar, but with lower TPR due to the disproportionately large effect of the heterogeneous covariate on the response\relax }}{29}{table.caption.3}\protected@file@percent }
\newlabel{Table1}{{2}{29}{\small True positive rates (TPR) and true negative rates (TNR) for variable selection averaged across simulations. The proposed approach ($\mbox {S}_{small}(\tau )$) neatly balances TPR and TNR. The Bayesian competitor ($\mbox {AL}_ {Bayes}$) is significantly underpowered due to excessively wide posterior credible intervals, while the frequentist competitor (aLASSO) often overselects variables (low TNRs). The results for the $(n,p) = (100,100)$ are qualitatively similar, but with lower TPR due to the disproportionately large effect of the heterogeneous covariate on the response\relax }{table.caption.3}{}}
\citation{miranda2007relationship,bravo2024spatial}
\citation{CEHI}
\citation{bravo2022racial}
\citation{bravo2022racial}
\@writefile{toc}{\contentsline {section}{\numberline {5}Social Stressors, Environmental Exposures, and Childhood Educational Outcomes}{30}{section.5}\protected@file@percent }
\newlabel{realdat}{{5}{30}{Social Stressors, Environmental Exposures, and Childhood Educational Outcomes}{section.5}{}}
\citation{gelman1996posterior}
\newlabel{tab:variable}{{\caption@xref {tab:variable}{ on input line 1302}}{31}{Social Stressors, Environmental Exposures, and Childhood Educational Outcomes}{table.caption.4}{}}
\@writefile{lot}{\contentsline {table}{\numberline {3}{\ignorespaces \small  Variables in the North Carolina dataset. Data are restricted to children with NH Black or NH White mothers \citep  {bravo2022racial}, 30-42 weeks of gestation, 0-104 weeks of age-within-cohort, mother's age 15-44, \texttt  {Blood\_Lead} $\leq $ 10, birth order $\leq $ 4, no status as an English language learner, and residence in NC at the time of birth and the time of 4th EoG test. Numeric covariates are centered and scaled to mean zero and standard deviation 0.5.\relax }}{31}{table.caption.4}\protected@file@percent }
\newlabel{tabdata}{{3}{31}{\small Variables in the North Carolina dataset. Data are restricted to children with NH Black or NH White mothers \citep {bravo2022racial}, 30-42 weeks of gestation, 0-104 weeks of age-within-cohort, mother's age 15-44, \texttt {Blood\_Lead} $\leq $ 10, birth order $\leq $ 4, no status as an English language learner, and residence in NC at the time of birth and the time of 4th EoG test. Numeric covariates are centered and scaled to mean zero and standard deviation 0.5.\relax }{table.caption.4}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces \small  Quantile-specific point estimates and 95\% credible intervals for main effects (not interacted with mother's race) under $\mbox  {S}_{small}$ (purple), $\mbox  {AL}_{Bayes}$ (green) and $\mbox  {aLASSO}$ (yellow); the horizontal line denotes zero. Under the proposed approach ($\mbox  {S}_{small}$), we identify several heterogeneous effects on reading scores, including gender and economically disadvantaged students. Other effects, such birthweight percentile and mother's age, are relatively homogeneous. By contrast, $\mbox  {AL}_{Bayes}$ exhibits excessively wide credible intervals, especially for extreme quantiles, while the $\mbox  {aLASSO}$ estimates are highly variable and nonsmooth across $\tau $.\relax }}{33}{figure.caption.5}\protected@file@percent }
\newlabel{main}{{2}{33}{\small Quantile-specific point estimates and 95\% credible intervals for main effects (not interacted with mother's race) under $\mbox {S}_{small}$ (purple), $\mbox {AL}_{Bayes}$ (green) and $\mbox {aLASSO}$ (yellow); the horizontal line denotes zero. Under the proposed approach ($\mbox {S}_{small}$), we identify several heterogeneous effects on reading scores, including gender and economically disadvantaged students. Other effects, such birthweight percentile and mother's age, are relatively homogeneous. By contrast, $\mbox {AL}_{Bayes}$ exhibits excessively wide credible intervals, especially for extreme quantiles, while the $\mbox {aLASSO}$ estimates are highly variable and nonsmooth across $\tau $.\relax }{figure.caption.5}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces \small  Quantile-specific point estimates and 95\% credible intervals for social and environmental exposures that are interacted with mother's race under $\mbox  {S}_{small}$ (purple), $\mbox  {AL}_{Bayes}$ (green) and $\mbox  {aLASSO}$ (yellow); the horizontal line denotes zero. The main effects (left) refer specifically to the NH White group, while the interaction effects (right) refer to the differences between these effects for NH Black students and NH White students. Under $\mbox  {S}_{small}(\tau )$, the \text  {\normalfont  \ttfamily  blood_lead} effects are increasingly negative for $\tau < 0.5$, with no clear differences between NH Black and NH White students. \text  {\normalfont  \ttfamily  RI} similarly exhibits an increasingly negative effect for lower quantiles, but only for NH Black students. Finally, the \text  {\normalfont  \ttfamily  NDI} effects are heterogeneous and increasingly negative for lower quantiles among NH White students, but for NH Black students, the effects are negative yet homogeneous across $\tau $. Again, $\mbox  {AL}_{Bayes}$ produces excessively wide credible intervals, while aLASSO only identifies nonzero effects for \text  {\normalfont  \ttfamily  NDI} among NH White students.\relax }}{34}{figure.caption.6}\protected@file@percent }
\newlabel{intrctt}{{3}{34}{\small Quantile-specific point estimates and 95\% credible intervals for social and environmental exposures that are interacted with mother's race under $\mbox {S}_{small}$ (purple), $\mbox {AL}_{Bayes}$ (green) and $\mbox {aLASSO}$ (yellow); the horizontal line denotes zero. The main effects (left) refer specifically to the NH White group, while the interaction effects (right) refer to the differences between these effects for NH Black students and NH White students. Under $\mbox {S}_{small}(\tau )$, the \vtt {blood_lead} effects are increasingly negative for $\tau < 0.5$, with no clear differences between NH Black and NH White students. \vtt {RI} similarly exhibits an increasingly negative effect for lower quantiles, but only for NH Black students. Finally, the \vtt {NDI} effects are heterogeneous and increasingly negative for lower quantiles among NH White students, but for NH Black students, the effects are negative yet homogeneous across $\tau $. Again, $\mbox {AL}_{Bayes}$ produces excessively wide credible intervals, while aLASSO only identifies nonzero effects for \vtt {NDI} among NH White students.\relax }{figure.caption.6}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces \small  Variable importance $\mbox  {VI}_{j}(\tau )$ from \eqref  {VI}, colored by quantile; the dashed line indicates 0.90. Large values indicate that the covariate appears in many of the acceptable subsets. \text  {\normalfont  \ttfamily  mEdu}, \text  {\normalfont  \ttfamily  mRace} and \text  {\normalfont  \ttfamily  EconDisadvantage} appear in all acceptable subsets for all quantiles, while several of the environmental and social factors exhibit heterogeneous variable importance, often with increasing $\mbox  {VI}_{j}(\tau )$ for smaller quantiles (See Section E.\relax }}{35}{figure.caption.7}\protected@file@percent }
\newlabel{vimps}{{4}{35}{\small Variable importance $\mbox {VI}_{j}(\tau )$ from \eqref {VI}, colored by quantile; the dashed line indicates 0.90. Large values indicate that the covariate appears in many of the acceptable subsets. \vtt {mEdu}, \vtt {mRace} and \vtt {EconDisadvantage} appear in all acceptable subsets for all quantiles, while several of the environmental and social factors exhibit heterogeneous variable importance, often with increasing $\mbox {VI}_{j}(\tau )$ for smaller quantiles (See Section E.\relax }{figure.caption.7}{}}
\@writefile{toc}{\contentsline {section}{\numberline {6}Conclusion}{36}{section.6}\protected@file@percent }
\newlabel{conclude}{{6}{36}{Conclusion}{section.6}{}}
\citation{pratola2020heteroscedastic}
\citation{fagnant2020characterizing}
\bibstyle{jasa3.bst}
\bibdata{reference}
\bibcite{alhamzawi2020brq}{{1}{2020}{{Alhamzawi and Ali}}{{Alhamzawi and Ali}}}
\@writefile{toc}{\contentsline {section}{\numberline {7}Acknowledgments}{38}{section.7}\protected@file@percent }
\bibcite{alhamzawi2012bayesian}{{2}{2012}{{Alhamzawi et~al.}}{{Alhamzawi, Yu, and Benoit}}}
\bibcite{bassett2002portfolio}{{3}{2002}{{Bassett and Chen}}{{Bassett and Chen}}}
\bibcite{10.1214/10-AOS827}{{4}{2011}{{Belloni and Chernozhukov}}{{Belloni and Chernozhukov}}}
\bibcite{benoit2017bayesqr}{{5}{2017}{{Benoit and Van~den Poel}}{{Benoit and Van~den Poel}}}
\bibcite{Bertsimas2006}{{6}{2016}{{Bertsimas et~al.}}{{Bertsimas, King, and Mazumder}}}
\bibcite{bondell2010noncrossing}{{7}{2010}{{Bondell et~al.}}{{Bondell, Reich, and Wang}}}
\bibcite{bravo2024spatial}{{8}{2024}{{Bravo et~al.}}{{Bravo, Kowal, Zephyr, Feldman, Ensor, and Miranda}}}
\bibcite{bravo2022racial}{{9}{2022}{{Bravo et~al.}}{{Bravo, Zephyr, Kowal, Ensor, and Miranda}}}
\bibcite{carpenter2017stan}{{10}{2017}{{Carpenter et~al.}}{{Carpenter, Gelman, Hoffman, Lee, Goodrich, Betancourt, Brubaker, Guo, Li, and Riddell}}}
\bibcite{CEHI}{{11}{2020}{{CEHI}}{{CEHI}}}
\bibcite{chen2013bayesian}{{12}{2013}{{Chen et~al.}}{{Chen, Dunson, Reed, and Yu}}}
\bibcite{dao2022bayesian}{{13}{2022}{{Dao et~al.}}{{Dao, Wang, Ghosh, and Ye}}}
\bibcite{dunson2005approximate}{{14}{2005}{{Dunson and Taylor}}{{Dunson and Taylor}}}
\bibcite{fagnant2020characterizing}{{15}{2020}{{Fagnant et~al.}}{{Fagnant, Gori, Sebastian, Bedient, and Ensor}}}
\bibcite{fasiolo2021fast}{{16}{2021}{{Fasiolo et~al.}}{{Fasiolo, Wood, Zaffran, Nedellec, and Goude}}}
\bibcite{frechet1948elements}{{17}{1948}{{Fr{\'e}chet}}{{Fr{\'e}chet}}}
\bibcite{furnival2000regressions}{{18}{2000}{{Furnival and Wilson}}{{Furnival and Wilson}}}
\bibcite{gelman1996posterior}{{19}{1996}{{Gelman et~al.}}{{Gelman, Meng, and Stern}}}
\bibcite{HahnCarvalho}{{20}{2015}{{Hahn and Carvalho}}{{Hahn and Carvalho}}}
\bibcite{hofmann2007efficient}{{21}{2007}{{Hofmann et~al.}}{{Hofmann, Gatu, and Kontoghiorghes}}}
\bibcite{Tokdar}{{22}{2012}{{Kadane and Tokdar}}{{Kadane and Tokdar}}}
\bibcite{keil2020quantile}{{23}{2020}{{Keil et~al.}}{{Keil, Buckley, O’Brien, Ferguson, Zhao, and White}}}
\bibcite{koenker1978regression}{{24}{1978}{{Koenker and Bassett~Jr}}{{Koenker and Bassett~Jr}}}
\bibcite{koenker2017handbook}{{25}{2017}{{Koenker et~al.}}{{Koenker, Chernozhukov, He, and Peng}}}
\bibcite{kottas2001bayesian}{{26}{2001}{{Kottas and Gelfand}}{{Kottas and Gelfand}}}
\bibcite{kottas2009bayesian}{{27}{2009}{{Kottas and Krnjaji{\'c}}}{{Kottas and Krnjaji{\'c}}}}
\bibcite{kowal2021fast}{{28}{2021}{{Kowal}}{{Kowal}}}
\bibcite{DKJMLR}{{29}{2022}{{Kowal}}{{Kowal}}}
\bibcite{kowal2024monte}{{30}{2024}{{Kowal and Wu}}{{Kowal and Wu}}}
\bibcite{kozumi2011gibbs}{{31}{2011}{{Kozumi and Kobayashi}}{{Kozumi and Kobayashi}}}
\bibcite{lee2014model}{{32}{2014}{{Lee et~al.}}{{Lee, Noh, and Park}}}
\bibcite{li20081}{{33}{2008}{{Li and Zhu}}{{Li and Zhu}}}
\bibcite{miranda2007relationship}{{34}{2007}{{Miranda et~al.}}{{Miranda, Kim, Galeano, Paul, Hull, and Morgan}}}
\bibcite{pandey1999comparative}{{35}{1999}{{Pandey and Nguyen}}{{Pandey and Nguyen}}}
\bibcite{PetersenAlexander2021W}{{36}{2021}{{Petersen et~al.}}{{Petersen, Liu, and Divani}}}
\bibcite{pratola2020heteroscedastic}{{37}{2020}{{Pratola et~al.}}{{Pratola, Chipman, George, and McCulloch}}}
\bibcite{raftery1997bayesian}{{38}{1997}{{Raftery et~al.}}{{Raftery, Madigan, and Hoeting}}}
\bibcite{reichBNPqr}{{39}{2009}{{Reich et~al.}}{{Reich, Bondell, and Wang}}}
\bibcite{reich2013bayesian}{{40}{2013}{{Reich and Smith}}{{Reich and Smith}}}
\bibcite{sherwood2017rqpen}{{41}{2017}{{Sherwood and Maidman}}{{Sherwood and Maidman}}}
\bibcite{ALconsist}{{42}{2013}{{Sriram et~al.}}{{Sriram, Ramamoorthi, and Ghosh}}}
\bibcite{taddy2010bayesian}{{43}{2010}{{Taddy and Kottas}}{{Taddy and Kottas}}}
\bibcite{wang2012quantile}{{44}{2012}{{Wang et~al.}}{{Wang, Wu, and Li}}}
\bibcite{woody}{{45}{2021}{{Woody et~al.}}{{Woody, Carvalho, and Murray}}}
\bibcite{wu2009variable}{{46}{2009}{{Wu and Liu}}{{Wu and Liu}}}
\bibcite{emplike}{{47}{2012}{{Yang and He}}{{Yang and He}}}
\bibcite{stacking}{{48}{2018}{{Yao et~al.}}{{Yao, Vehtari, Simpson, and Gelman}}}
\bibcite{yu2001bayesian}{{49}{2001}{{Yu and Moyeed}}{{Yu and Moyeed}}}
\gdef \@abspage@last{44}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> xx.tex <==


